Explicable hyper-reduced order models on nonlinearly approximated solution manifolds of compressible and incompressible Navier-Stokes equations

A slow decaying Kolmogorov n-width of the solution manifold of a parametric partial differential equation precludes the realization of efficient linear projection-based reduced-order models. This is due to the high dimensionality of the reduced space needed to approximate with sufficient accuracy the solution manifold. To solve this problem, neural networks, in the form of different architectures, have been employed to build accurate nonlinear regressions of the solution manifolds. However, the majority of the implementations are non-intrusive black-box surrogate models, and only a part of them perform dimension reduction from the number of degrees of freedom of the discretized parametric models to a latent dimension. We present a new intrusive and explicable methodology for reduced-order modelling that employs neural networks for solution manifold approximation but that does not discard the physical and numerical models underneath in the predictive/online stage. We will focus on autoencoders used to compress further the dimensionality of linear approximants of solution manifolds, achieving in the end a nonlinear dimension reduction. After having obtained an accurate nonlinear approximant, we seek for the solutions on the latent manifold with the residual-based nonlinear least-squares Petrov-Galerkin method, opportunely hyper-reduced in order to be independent from the number of degrees of freedom. New adaptive hyper-reduction strategies are developed along with the employment of local nonlinear approximants. We test our methodology on two nonlinear time-dependent parametric benchmarks involving a supersonic flow past a NACA airfoil with changing Mach number and an incompressible turbulent flow around the Ahmed body with changing slant angle.

==> sections/airfoil.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1\textwidth, trim={200 100 200 0}, clip]{figures/mp_convergence.pdf}
  \caption{Comparison of methodologies after time step $800$}
\end{figure}

==> sections/mor.tex <==
In this section, we want to write a reduced order model (ROM) for the FS in case of parameter dependent problems \cite{hesthaven2016certified,rozza2022advanced}.
To do so, we exploit two aspects of the above presented FS: the linearity of the problems and the affine dependence of the operators on the parameters.

As we have seen in Section \ref{sec:examples}, all the problems are depending on some parameters $\rho \in\mathcal{P} \subset \R^{\Npar}$ and the dependence is affine. 
This means that it is possible to find $\Naff$ terms independent on the parameters for each form, such that they can be affinely combined to obtain the original operator, i.e.,
\begin{equation}
	a_h(z,y_h;\rho) = \sum_{\ell=1}^{\Naff} \theta_\ell^a(\rho) a_{\ell,h}(z,y_h), \qquad l_h(y_h) = \sum_{\ell=1}^{\Naff} \theta_\ell^f(\rho) l_{h, l}(y_h).
\end{equation}

Then, we select a reduced space $V_\NRB\subset V_h$ provided by a compression algorithm, e.g. POD/PCA \cite{jolliffe2002principal,kunisch2001galerkin,torlo2021model} or Greedy algorithm \cite{prud2002mathematical,prud2002reliable,hesthaven2016certified,crisovan2019model}. We suppose that the reduced dimension $\NRB$ is much smaller than the dimension $\NDG$ of the full order model space $V_h$. 
We look for a reduced solution $\zRB\in V_\NRB$ as a linear combination of the bases $\lbrace \psiRB_j\rbrace_{j=1}^{\NRB} $ of $ V_\NRB$, i.e.,
\begin{equation}
	\zRB = \sum_{j=1}^{\NRB} \zRB^j \psiRB_j.
\end{equation}
Performing a standard Galerkin projection we obtain the following $\RB$ problem.
\begin{definition}[Reduced Basis Problem]
	Find $\zRB\in V_\NRB$, given by the coefficients $\zRB^j$, such that 
	\begin{equation}
		\sum_{i=1}^{\NRB} \zRB^j(\rho) \sum_{\ell=1}^{\Naff} \theta_\ell^a(\rho) a_{\ell,h}(\psiRB_j,\psiRB_i) = \sum_{\ell=1}^{\Naff}\theta_\ell^f(\rho)(f_\ell,\psiRB_i), \qquad \text{for all }i=1,\dots, \NRB. 
	\end{equation}
\end{definition}
The obtained problem scales depend on the dimension $\NRB$ and $\Naff$ in its assembly and only on $\NRB$ in its solution, and it is completely independent on $\NDG$.
To obtain computational advantages for the parametric problem, we split the tasks into an expensive \textit{offline phase } and a cheap online phase. 
In the \textit{offline phase}, we find the reduced space $V_\NRB$ and we assemble the reduced matrices and right hand sides 
\begin{equation}
	A_\ell:=\lbrace a_{\ell,h}(\psiRB_j,\psiRB_i) \rbrace_{i,j}, \qquad b_\ell:=\lbrace (f_\ell,\psiRB_i)\rbrace_{i}.
\end{equation}
In the \textit{online phase}, we can simply evaluate the coefficients $\theta^a_\ell(\rho)$ and $\theta^f_\ell(\rho)$ and obtain the reduced linear system
\begin{equation}
	A(\rho)z_{\RB} = b(\rho), \qquad \text{with } A(\rho):=\sum_\ell\theta^a_\ell(\rho) A_\ell \text{ and }b(\rho):= \sum_\ell\theta^f_\ell(\rho) b_\ell.
\end{equation}
This gives a great speedup in computational times.

% \subsection{Compression algorithms}
% The reduced space $V_\NRB$ can be obtained with different techniques. 
% The goal is to minimize the approximation error
% \begin{equation}
% 	\left\lVert  z_h(\rho)-\Pi_{\RB}(z_h(\rho)) \right\rVert
% \end{equation}
% for $\rho \in \mathcal{P}$, with $\Pi_{\RB}$ being the projection onto $V_\NRB$.
% Two of the most classical and popular ones are the proper orthogonal decomposition (POD) \cite{kunisch2001galerkin,jolliffe2002principal} and the Greedy algorithm \cite{prud2002mathematical,prud2002reliable}.

% The POD considers a training set of parameters $\lbrace \rho_i \rbrace_{i=1}^{\Ntrain}$, 
% computes the FOM solution for all the parameters $\lbrace{ z_h(\rho_i)}\rbrace_{i=1}^{\Ntrain}$ 
% and builds the snapshot matrix by juxtaposition of the snapshots. It computes the economic SVD 
% of the snapshot matrix and selects the most relevant values according to a tolerance or a number 
% of basis $\NRB$. The corresponding singular vectors provides the basis of the reduced space.
% The advantage of the POD is that it provides a reliable measure of the approximation error in $L^2$ of the training set \cite{kunisch2001galerkin}. 
% The drawback consists of the computation of the FOM for all the parameters in the training set.

% The Greedy algorithm is an iterative procedure that at each step selects the \textit{worst represented} parameter in the training set, computes the FOM solution of this parameter and increase the reduced basis by this snapshot. 
% The algorithm stops when the worst error is below a certain tolerance.
% The advantage of the Greedy method is that only few FOM solutions are computed along the process, the difficult part is to have a good and cheap estimator of the error that allows to choose the \textit{worst represented} parameter without computing the FOM solution.
% In order to do so, different error estimators have been developed for different problems in literature \cite{prud2002mathematical,prud2002reliable}, but not always is possible to obtain a reliable and cheap error estimator.

% In the next section, we provide an error bound for FS. In the test section, we will compare both algorithms.

